Peer2PIR: Private Queries for IPFS

The InterPlanetary File System (IPFS) is a peer-to-peer network for storing data in a distributed file system, hosting over 190,000 peers spanning 152 countries. Despite its prominence, the privacy properties that IPFS offers to peers are severely limited. Any query within the network leaks the queried content to other peers. We address IPFS' privacy leakage across three functionalities (peer routing, provider advertisements, and content retrieval), ultimately empowering peers to privately navigate and retrieve content in the network. Our work highlights and addresses novel challenges inherent to integrating PIR into distributed systems. We present our new, private protocols and demonstrate that they incur reasonably low communication and computation overheads. We also provide a systematic comparison of state-of-art PIR protocols in the context of distributed systems.

==> conclusion.tex <==
\section{Conclusion}
\label{sec.conclusion}

We address the problem of a peer privately retrieving content and routing information from other peers within IPFS.
We provide three scalable algorithms to enable a peer to privately retrieve routes to another peer, discover peers providing desired content, and fetch this content from these peers.
We integrate our algorithms within the IPFS design, ensuring that they handle constraints unique to it.
Our algorithms rely on private information retrieval protocols, and so we systematically analyze how recent protocols can handle the three aforementioned problems.
We propose two PIR protocols that combine techniques from cryptographic folklore and address a gap in the design space. 
Finally, we evaluate the correctness and overheads of our algorithms.
We hope that our work inspires further research into the privacy and security challenges within IPFS and P2P systems.
